A Domain-Specific Language for Rich Motor Skill Architectures

Model-driven software development is a promising way to cope with the complexity of system integration in advanced robotics, as it already demonstrated its benefits in domains with comparably challenging system integration requirements. This paper reports on work in progress in this area which aims to improve the research and experimentation process in a collaborative research project developing motor skill architectures for compliant robots. Our goal is to establish a model-driven development process throughout the project around a domain-specific language (DSL) facilitating the compact description of adaptive modular architectures for rich motor skills. Incorporating further languages for other aspects (e.g. mapping to a technical component architecture) the approach allows not only the formal description of motor skill architectures but also automated code-generation for experimentation on technical robot platforms. This paper reports on a first case study exemplifying how the developed AMARSi DSL helps to conceptualize different architectural approaches and to identify their similarities and differences.

==> tex/process.tex <==
\textbf{Short description of how we want to embed the DSLs in our MDSD process, Fig.~\ref{fig:mdsd} (chapter may be subject to kuerzung)}

MDSD establishes an engineering process, linked to ongoing research in software engineering (for robotics)

Eases communication and understanding between partners, work-packages and across disciplines

Architecture-centric, generative approach. Clear separation of concerns. Allows quantitative and qualitative validation

Allows scientific analysis of system and components

\begin{figure}[t]
 \centering
 \includegraphics[width=.35\textwidth]{MDSD-Process}
 \caption{Model-Driven Software Development Process}
 \label{fig:mdsd}
\end{figure}

\bitem{}
\item Code generation: Domain-specific programming model of the AMARSi
\item Compliant Control Architecture (CCA)
\item Mapping of the DSL concepts to programming / system-level elements
\item E.g., Component with Ports, Buffers, and Spaces
\eitem{}

